Dynamic Adapter with Semantics Disentangling for Cross-lingual Cross-modal Retrieval

Existing cross-modal retrieval methods typically rely on large-scale vision-language pair data. This makes it challenging to efficiently develop a cross-modal retrieval model for under-resourced languages of interest. Therefore, Cross-lingual Cross-modal Retrieval (CCR), which aims to align vision and the low-resource language (the target language) without using any human-labeled target-language data, has gained increasing attention. As a general parameter-efficient way, a common solution is to utilize adapter modules to transfer the vision-language alignment ability of Vision-Language Pretraining (VLP) models from a source language to a target language. However, these adapters are usually static once learned, making it difficult to adapt to target-language captions with varied expressions. To alleviate it, we propose Dynamic Adapter with Semantics Disentangling (DASD), whose parameters are dynamically generated conditioned on the characteristics of the input captions. Considering that the semantics and expression styles of the input caption largely influence how to encode it, we propose a semantic disentangling module to extract the semantic-related and semantic-agnostic features from the input, ensuring that generated adapters are well-suited to the characteristics of input caption. Extensive experiments on two image-text datasets and one video-text dataset demonstrate the effectiveness of our model for cross-lingual cross-modal retrieval, as well as its good compatibility with various VLP models.

==> checklist.tex <==

\section{Reproducibility Checklist}
\begin{enumerate}
\item This paper:
    \begin{itemize}
        \item  Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes/partial/no/NA)
        yes
        \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes/no)
        yes
        \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes/no)
        yes
    \end{itemize}
\item Does this paper make theoretical contributions? (yes/no)
yes

If yes, please complete the list below.
    \begin{itemize}
        \item All assumptions and restrictions are stated clearly and formally. (yes/partial/no)
        yes
        \item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)
        yes
        \item Proofs of all novel claims are included. (yes/partial/no)
        yes
        \item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)
        yes
        \item Appropriate citations to theoretical tools used are given. (yes/partial/no)
        yes
        \item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)
        yes
        \item All experimental code used to eliminate or disprove claims is included. (yes/no/NA)
        yes
    \end{itemize}
\item Does this paper rely on one or more datasets? (yes/no)
yes

If yes, please complete the list below.
    \begin{itemize}
        \item A motivation is given for why the experiments are conducted on the selected datasets (yes/partial/no/NA)
        yes
        \item All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA)
        NA
        \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA)
        NA
        \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes/no/NA)
        yes
        \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes/partial/no/NA)
        yes
        \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/NA)
        NA
    \end{itemize}
\item Does this paper include computational experiments? (yes/no)
yes


If yes, please complete the list below.

    \begin{itemize}
        \item Any code required for pre-processing data is included in the appendix. (yes/partial/no).
        yes
        \item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no)
        yes
        \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no)
        yes
        \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes/partial/no)
        yes
        \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA)
        yes
        \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no)
        yes
        \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no)
        yes
        \item This paper states the number of algorithm runs used to compute each reported result. (yes/no)
        yes
        \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no)
        yes
        \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no)
        yes
        \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes/partial/no/NA)
        yes
        \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA)
        yes

    \end{itemize}

\end{enumerate}
